The Sketching Complexity of Graph and Hypergraph Counting

Subgraph counting is a fundamental primitive in graph processing, with applications in social network analysis (e.g., estimating the clustering coefficient of a graph), database processing and other areas. The space complexity of subgraph counting has been studied extensively in the literature, but many natural settings are still not well understood. In this paper we revisit the subgraph (and hypergraph) counting problem in the sketching model, where the algorithm's state as it processes a stream of updates to the graph is a linear function of the stream. This model has recently received a lot of attention in the literature, and has become a standard model for solving dynamic graph streaming problems. In this paper we give a tight bound on the sketching complexity of counting the number of occurrences of a small subgraph $H$ in a bounded degree graph $G$ presented as a stream of edge updates. Specifically, we show that the space complexity of the problem is governed by the fractional vertex cover number of the graph $H$. Our subgraph counting algorithm implements a natural vertex sampling approach, with sampling probabilities governed by the vertex cover of $H$. Our main technical contribution lies in a new set of Fourier analytic tools that we develop to analyze multiplayer communication protocols in the simultaneous communication model, allowing us to prove a tight lower bound. We believe that our techniques are likely to find applications in other settings. Besides giving tight bounds for all graphs $H$, both our algorithm and lower bounds extend to the hypergraph setting, albeit with some loss in space complexity.

==> illustration.tex <==
\section{Illustration of Communication Problem}

\begin{figure}
  \centering
    \begin{subfigure}[t]{0.47\textwidth}
            \centering
            \includegraphics[width=\textwidth]{illustration1}
            \caption{Input for triangle-counting when all permutations
              are identity.  Each player $e$ sees $n$ edges with
              associated binary labels (pictured as solid/dashed).
              The edges match up into $T$ triangles (center) and $n-T$
              isolated edges (outside).  The goal is to determine
              whether every triangle has an even number of solid
              edges, or an odd number.}
            \label{fig:fig1}
    \end{subfigure}\hfill
\begin{subfigure}[t]{0.47\textwidth}
            \centering
            \includegraphics[width=\textwidth]{illustration2}
            \caption{In the hard distribution, we randomly permute the
              vertices on top, on left, and on right.  Each player
              sees their edges, with associated labels, in a random
              order.}
    \label{fig:fig2}
    \end{subfigure}
    \caption{Lower bound instance for triangle counting}
\end{figure}

